Zak-OTFS for Mutually Unbiased Sensing and Communication

Waveforms with ideal ambiguity functions are fundamental to integrated sensing and communication, to active sensing (radar), and to uplink multiple access. We describe a general method of constructing waveforms using the discrete Zak transform (DZT) to convert sequences of length $MN$ in the time domain to waveforms in the delay-Doppler (DD) domain, each of which is defined by an $M\times N$ quasi-periodic array. The DZT preserves inner products, and we show that phase coded waveforms used in radar (CAZAC sequences) determine noise-like waveforms in the DD domain, each with low Peak to Average Power Ratio. In a Zak-OTFS communication system, we show that these waveforms are mutually unbiased with respect to every carrier and use them to integrate sensing and communication as spread pilots. We view each waveform as a linear combination of Zak-OTFS carriers and show that the self-ambiguity function is supported on a discrete line in the integers modulo $MN$. The sidelobes are significantly lower than the original CAZAC sequence, and the advantage of discrete support is better localization/resolution in delay and Doppler compared with standard methods based on chirps or tones. We show that the absolute value of the cross-ambiguity function for pairs of waveforms in the same family is small and constant. This property makes the waveforms ideal preambles in the 2-step RACH protocol introduced in Release 15, 3GPP to enable grant-free multiple access. The characteristics of the cross-ambiguity function make it possible to simultaneously detect multiple preambles in the presence of mobility and delay spread.

==> ProofDDFilter.tex <==
\section{Self-Ambiguity of General CAZAC DD Filter}

We define an general CAZAC filter in the delay-Doppler domain as a function of the roots of unity:
\begin{align}
    \label{eq:ddfiltercazac}
    \mathbf{W}[k,l] = e^{j2\pi\frac{\alpha_{1} k^2 + \beta_{1} k + \alpha_{2} l^2 + \beta_{2} l + \gamma}{MN}},~\forall k,l \in \mathbb{Z},
\end{align}
where $\alpha_{1}, \alpha_{2}, \beta_{1}, \beta_{2}, \gamma \in \mathbb{Z}$. Note that $\mathbf{W}[k,l]$ has period $MN$ in both $k$ and $l$. Note that when $\alpha_{1} = \alpha_{2} = q$ and $\beta_{1} = \beta_{2} = \gamma = 0$,~\eqref{eq:ddfiltercazac} reduces to the discrete chirp filter defined in~\cite{Aug2024paper}.

The DD domain spread pilot $x_{s}[k,l]$ is generated by filtering a point pilot $x_{p}[k,l]$ as~\cite{Aug2024paper}:
\begin{align}
    \label{eq:ddspreadpilot}
    x_{s}[k,l] = \mathbf{W}[k,l] \circledast_{\sigma} x_{p}[k,l],
\end{align}
where $\circledast_{\sigma}$ denotes discrete-domain $(MN)$-periodic twisted convolution~\cite{Aug2024paper},
\begin{align}
    \label{eq:twistedconvdiscrete}
    &a[k,l] \circledast_{\sigma} b[k,l] \nonumber \\ &= \sum_{k',l' \in \mathbb{Z}}\!a[k',l'] b[k-k',l-l'] e^{j 2\pi \frac{l'(k-k')}{MN}},
\end{align}
for $(MN)$-periodic $a[k,l]$ and quasi-periodic $b[k,l]$, and $x_{p}[k,l]$ is the quasi-periodic point pilot at $(k_{p},l_{p})$~\cite{Aug2024paper}:
\begin{align}
    \label{eq:ddpointpilot}
    x_{p}[k,l]\!=\!\sum_{n,m \in \mathbb{Z}}\!e^{j 2\pi \frac{nl}{N}} \delta[k-k_{p}-nM] \delta[l-l_{p}-mN].
\end{align}

For simplicity, in the remainder of this Section, we consider $(k_{p},l_{p}) = (0,0)$ in~\eqref{eq:ddpointpilot}, for which~\eqref{eq:ddspreadpilot} simplifies to~\cite{Aug2024paper}
\begin{align}
    \label{eq:ddspreadpilotsimp}
    x_{s}[k,l] = \sum_{n = 0}^{N-1} \sum_{m = 0}^{M-1} \mathbf{W}[k-nM,l-mN] e^{j 2\pi \frac{nl}{N}}.
\end{align}

The self-ambiguity function per~\eqref{eq:amb} of $\mathbf{X}[k,l] = x_{s}[k,l]$ is:
\begin{align}
    \label{eq:ddfilteramb1}
    \mathbf{A}[k,l] &= \frac{1}{MN} \sum_{k'=0}^{M-1} \sum_{l'=0}^{N-1} \sum_{n=0}^{N-1} \sum_{n'=0}^{N-1} \sum_{m=0}^{M-1} \sum_{m'=0}^{M-1} e^{j \frac{2\pi}{MN} \mathsf{B}}, \nonumber \\
    \mathsf{B} &= (nl' - n'(l'-l)) M - (k'-k)l + \alpha_{1} (k'-nM)^{2} \nonumber \\ &+ \alpha_{2} (l'-mN)^{2} + \beta_{1} (k'-nM) + \beta_{2} (l'-mN) \nonumber \\ &- \alpha_{1} (k'-k-n'M)^{2} - \alpha_{2} (l'-l-m'N)^{2} \nonumber \\ &- \beta_{1} (k'-k-n'M) - \beta_{2} (l'-l-m'N) \nonumber \\ &= n'Ml + kl - \alpha_{1}(k+(n'-n)M)(k+(n'+n)M) \nonumber \\ & - \alpha_{2}(l+(m'-m)N)(l+(m'+m)N) + \beta_{1} k + \beta_{2} l +\nonumber \\ &\beta_{1}(n'-n)M + l' \big[(n-n')M + 2\alpha_{2}(l+(m'-m)N)\big]\nonumber \\ &+\!\beta_{2}(m'-m)N\!+\!k'\big[2\alpha_{1}(k+(n'-n)M-l\big].
\end{align}

Thus, the self-ambiguity can be written as: 
\begin{align}
    \label{eq:ddfilteramb2}
    \mathbf{A}[k,l] &= \sum_{n=0}^{N-1} \sum_{n'=0}^{N-1} \sum_{m=0}^{M-1} \sum_{m'=0}^{M-1} e^{j \frac{2\pi}{MN} \mathsf{C}} \times \nonumber \\ & \bigg(\frac{1}{M} \sum_{k'=0}^{M-1} e^{j \frac{2\pi}{MN} \mathsf{D} k'} \bigg) \bigg(\frac{1}{N} \sum_{l'=0}^{N-1} e^{j \frac{2\pi}{MN} \mathsf{E} l'} \bigg), \nonumber \\ \mathsf{C} &= \mathsf{B} - \mathsf{D} k' - \mathsf{E} l',\nonumber \\ \mathsf{D} &= 2\alpha_{1}(k+(n'-n)M-l, \nonumber \\ \mathsf{E} &= (n-n')M + 2\alpha_{2}(l+(m'-m)N).
\end{align}

Via the identity:
\begin{align}
    \label{eq:rootsofunitysum}
    \frac{1}{N}\sum_{n=0}^{N-1}e^{\frac{j2\pi}{N}\mathsf{X}n} = \begin{cases}
        1 \quad \text{if } \ \mathsf{X} \equiv 0 \mod (N) \\
        0 \quad \ \text{otherwise}
    \end{cases},
\end{align}
the ambiguity function in~\eqref{eq:ddfilteramb2} has non-zero magnitude when
\begin{align}
    \label{eq:ddfilterlattice1}
    \mathsf{D} &= 2\alpha_{1}(k+(n'-n)M-l \equiv 0 \mod (MN), \\
    \label{eq:ddfilterlattice2}
    \mathsf{E} &= (n-n')M + 2\alpha_{2}(l+(m'-m)N) \equiv 0 \mod (MN).
\end{align}

From~\eqref{eq:ddfilterlattice1}, we obtain
\begin{align}
    \label{eq:ddfilterlattice3}
    (n'-n)M \equiv ((2\alpha_{1})^{-1} l - k) \mod (MN).
\end{align}

Substituting~\eqref{eq:ddfilterlattice3} into~\eqref{eq:ddfilterlattice2}, we obtain
\begin{align}
    \label{eq:ddfilterlattice4}
    &2\alpha_{2}(m'-m)N \equiv \theta l - k \mod (MN), \nonumber \\ 
    &\theta = ((2\alpha_{1})^{-1} - 2\alpha_{2}) \mod (MN),
\end{align}
or equivalently when
\begin{align}
    \label{eq:ddfilterlattice5}
    2\alpha_{1} k - l &\equiv 0 \mod (M), \nonumber \\
    k - \theta l &\equiv 0 \mod (N).
\end{align}

Thus, the ambiguity function magnitude in~\eqref{eq:ddfilteramb2} is:
\begin{align}
    \vert\mathbf{A}[k, l]\vert = \begin{cases}
        1 \quad \ \text{if } \ \eqref{eq:ddfilterlattice5} \text{ is true} \\
        0 \quad \ \text{otherwise}
    \end{cases}.
    \label{eq:amb_abs_final}
\end{align}
This implies that for a general DD domain CAZAC filtered point pilot, its self-ambiguity is supported on a lattice in the DD domain. \hfill $\blacksquare$\\

==> data_preamble_crossamb.tex <==
\section{Mutually Unbiased Sensing \\ \& Communication Waveforms}
\label{sec:unbiased}

We now prove that the DD sequences $\mathbf{X}[k,l]$ constructed in~\eqref{eq:cazac_dd} are \emph{unbiased} to Zak-OTFS carrier waveforms used for communication in~\cite{bitspaper1,bitspaper2}. Within the fundamental period $\mathcal{D}_{0}$ (see Fig.~\ref{fig:pointpulsone} and~\cite{bitspaper1,bitspaper2,preamblepaper} for more details), the communication waveform is the sum of $MN$ information symbols: $\mathbf{D}[k,l] = \sum_{k_{p} = 0}^{M-1} \sum_{l_{p} = 0}^{N-1} x[k_{p},l_{p}] \delta[k-k_{p}] \delta[l-l_{p}]$. Per Definition~\ref{def:ddamb}, the cross-ambiguity between $\mathbf{D}[k,l]$ and $\mathbf{X}[k,l]$ evaluates to:
\begin{align}
    \label{eq:unbiased1}
    \mathbf{A}_{\mathbf{D},\mathbf{X}}[k,l] &= \frac{1}{MN^{\frac{3}{2}}} \sum_{k' = 0}^{M-1} \sum_{l' = 0}^{N-1} \sum_{k_{p} = 0}^{M-1} \sum_{l_{p} = 0}^{N-1} x[k_{p},l_{p}] \delta[k'-k_{p}] \delta[l'-l_{p}] \nonumber \\
    &\times e^{-\frac{j2\pi}{MN}\left(\gamma + (k'-k)\beta\right)} \sum_{p=0}^{N-1}e^{-\frac{j2\pi}{MN}\left(\alpha(k'-k+pM)^2+pM(\beta-l'+l)\right)} \nonumber \\ 
    &\times e^{-\frac{j2\pi}{MN} l(k'-k)} \nonumber \\
    &= \frac{1}{MN^{\frac{3}{2}}} \sum_{k_{p} = 0}^{M-1} \sum_{l_{p} = 0}^{N-1} x[k_{p},l_{p}] e^{-\frac{j2\pi}{MN}\left(\gamma + (k_{p}-k)(\beta+l)\right)} \nonumber \\ 
    &\times \sum_{p=0}^{N-1}e^{-\frac{j2\pi}{MN}\left(\alpha(k_{p}-k+pM)^2+pM(\beta-l_{p}+l)\right)} \nonumber \\
    &= \frac{1}{MN} \sum_{k_{p} = 0}^{M-1} \sum_{l_{p} = 0}^{N-1} x[k_{p},l_{p}] e^{-\frac{j2\pi}{MN}\left(\gamma + (k_{p}-k)(\beta+l)\right)} \nonumber \\ 
    &\times j \bigg(\frac{M}{N}\bigg) e^{-\frac{j2\pi}{N} (2nM + 2(k_{p}-k) + \beta - l_{p} + l)^{2} \psi(M)},
\end{align}
where $\psi(M) = (4M)^{-1}\mod (N)$.

The squared absolute value of~\eqref{eq:unbiased1} is:
\begin{align}
    \label{eq:unbiased2}
    \vert\mathbf{A}_{\mathbf{D},\mathbf{X}}[k,l]\vert^{2} &= \frac{1}{(MN)^{2}} \sum_{k_{p} = 0}^{M-1} \sum_{l_{p} = 0}^{N-1} \sum_{k'_{p} = 0}^{M-1} \sum_{l'_{p} = 0}^{N-1} x^{*}[k_{p},l_{p}] x[k'_{p},l'_{p}] \nonumber \\
    &e^{\frac{j2\pi}{MN} ((k_{p}-k'_{p})\beta +\alpha((k_{p}-k)^2 - (k'_{p}-k)^2) + l(k_{p}-k'_{p}))} \nonumber \\
    &e^{\frac{j2\pi}{N} 2(k_{p}-k'_{p}-l_{p}+l'_{p}) \psi(M)} = \frac{1}{MN},
\end{align}
where the final expression follows from the assumption that the information symbols $x[k_{p},l_{p}]$ are independent and identically distributed with unit energy.

Therefore, the cross-ambiguity function has magnitude $\vert\mathbf{A}_{\mathbf{D},\mathbf{X}}[k,l]\vert = \frac{1}{\sqrt{MN}}$, in other words, the sensing and communication waveforms are mutually unbiased. \hfill $\blacksquare$
